Artifacts in incomplete data tomography - with applications to photoacoustic tomography and sonar

We develop a paradigm using microlocal analysis that allows one to characterize the visible and added singularities in a broad range of incomplete data tomography problems. We give precise characterizations for photo- and thermoacoustic tomography and Sonar, and provide artifact reduction strategies. In particular, our theorems show that it is better to arrange Sonar detectors so that the boundary of the set of detectors does not have corners and is smooth. To illustrate our results, we provide reconstructions from synthetic spherical mean data as well as from experimental photoacoustic data.

==> characterization.tex <==

\section{Characterization of Limited Data Artifacts in PAT/TAT and
Sonar}
\label{sect:characterization} 

Using the paradigm of section \ref{sect:general strategy}, we now
describe the visible and added singularities for photo- and
thermoacoustic tomography (PAT and TAT, respectively), and sonar with
constant sound speed.  Proofs will be given in the appendix.

The same arguments can be used to prove the theorems in
\cite{FrikelQuinto2013} about limited angle tomography, even for the
generalized X-ray transform in the plane with arbitrary smooth
measures.  The arguments in \cite{FrikelQuinto2013,Katsevich:1997}
are more elementary and do not require the theory of FIO, but they do
not apply to generalized transforms.

\begin{remark}\label{remark:generalized}
Although we state the theorems for the circular and spherical
transforms with standard measures, our theorems are valid more
generally.  Theorems \ref{thm:visible and added sing} and
\ref{thm:reduction:circle} are valid for the generalized circular mean
transform with a smooth nowhere zero weight $\mu(\phi,x)\d x$ in
\eqref{def:Mc:circle}.  Theorems \ref{thm:visible and added sing
sphere} and \ref{thm:reduction:sphere} are valid for the generalized
circular mean transform with a smooth nowhere zero weight $\mu(y,x)\d
x$ in \eqref{def:Ms}.  In fact, our theorems are valid for any FIO
associated to the same canonical relation since our proofs use only
the properties of the operators as FIO and their associated their
canonical relations (when the operators can be composed).
\end{remark}

 \subsection{Photo- and thermoacoustic tomography for planar data
(circular Radon transform)}\label{sect:TAT}


In this section, we consider the so-called circular mean Radon
transform in 2D, which is a standard model for sectional imaging
setups of photoacoustic tomography with constant sound speed. We refer
to \cite{Elbau:2012df,
HaltmeierSchusterScherzer2005,KuchmentKunyanski2010} for overviews of
the mathematics behind PAT and TAT.  The forward transform is defined
by \bel{def:Mc} \Mc f(\xi,r) = \frac{1}{2\pi}\int_{u\in S^1}
f(\xi+ru)\d u,\quad (\xi,r)\in S\times (0,\infty),
\end{equation}
where $S$ is a smooth curve in $\R^2$. 

We will consider only functions and distributions on $\rtwo$ that are
supported inside the open unit disk $D=\sparen{x\in \rtwo\st \norm{x}<
1}$.  We will assume the detectors are on the circle $S=S^1$, and use
the parameterizations for vectors in $S^1$ and for circles
respectively
\[\th(\phi)=(\cos\phi,\sin\phi) \text{ for }\phi\in [0,2\pi],\quad
C(\phi,r) = \sparen{x\in \rtwo\st \norm{x-\th(\phi)}=r}.\] The
tomographic data will have the following parametrization
\bel{def:Mc:circle}\text{for }\ (\phi,r)\in
\Xi: = [0,2\pi]\times (0,\infty), \quad g(\phi,r)=\Mc
f(\phi,r):=\frac{1}{2\pi r}\int_{x\in C(\phi,r)} f(x)\d x,\ee where we identify
$0$ and $2\pi$ or, equivalently, consider only functions and
distributions on $\Xi$ that are $2\pi$ periodic in $\phi$.  Note that
the measure $\d x$ in this integral is the arc length measure. 

Then, the dual transform to $\Mc$ (using the standard measures on $D$
and $\Xi$) is \[\Mst g(x) = \int_{0}^{2\pi}
g(\phi,\norm{x-\th(\phi)})\frac{1}{2\pi \norm{x-\th(\phi)}}\d \phi.\]

Because $D$ is the open disk with boundary $S^1$, $\Mc:\Dc(D)\to
\Dc(\Xi)$ is continuous.  Therefore, its adjoint, $\Mst:\Dc'(\Xi)\to
\Dc'(D)$ is weakly continuous.  Similarly, $\Mc:\Ec'(D)\to \Ec'(\Xi)$
is weakly continuous.  


We will consider the limited data problem for this transform
specifying circular means with centers $\th(\phi)$ for $\phi \in
[a,b]$ with $b-a<2\pi$.  We define
\begin{equation}
\label{eq:restricted spherical mean transform} 
  \Mc_{[a,b]} f =
\chi_{A}\cdot\Mc f\ \ \text{ where $A=[a,b]\times (0,\infty)$}\,.
\end{equation}
  The wavefront
of $\chi_{A}$ is given by
\begin{equation}
\label{eq:WF hard cutoff} \WF(\chi_A) =
\sparen{((\phi,r),\nu\dphi)\st
\phi\in\sparen{a,b},\nu\neq0,r>0}.
\end{equation}

Before we state the main theorem of the section, we need to define
several concepts related to the microlocal analysis of the circular
mean transform.  For $\phi\in[0,2\pi]$ and $x\in D$, let
\bel{def:n}\npx = \frac{x-\th(\phi)}{\norm{x-\th(\phi)}}\,.\ee Then
$\npx$ the outward unit normal vector at $x$ to the circle
$C(\phi,\norm{x-\th(\phi)})$ centered at $\th(\phi)$ and containing
$x$. 


For $A\subset [0,2\pi]$ we define the set \bel{def:Va} \Vc_A :=
\sparen{(x,\xi\dx)\in T^*(D)\st \exists \phi\in A,\exists \alpha \neq
0, \xi = \alpha\npx}.\ee In our next theorem, we show $\Vab$
is the set of \emph{possible visible singularities}, i.e., those that
can be imaged by $\Mst P \Mab $ (singularities for $\phi\in
\sparen{a,b}$ might be cancelled).

For $f\in \Ec'(D)$, we define the set \bel{def:Aab}\begin{aligned}
\Aab(f):=&\big\{(x,\xi\dx)\in T^*(D)\st \exists \phi\in \sparen{a,b}\exists r\in
(0,2),\exists \alpha\neq 0, \\&\qquad
\exists \tx\in C(\phi,r)\cap D,\
\paren{\tx,\alpha\n(\phi,\tx)\dx}\in WF(f)\\
&\qquad \qquad\text{ and }x\in C(\phi,r)\cap D, \xi=\alpha\n(\phi,x)
\big\}.\end{aligned}\ee The set $\Aab(f)$ will include \emph{added
artifacts} in the reconstruction operator $\Mst P \Mab (f)$.


\begin{theorem}[Visible and Added Singularities]\label{thm:visible and
added sing}  Let $f\in \Ec'(D)$
and let $P$ be a pseudo\-differential operator on $\Dc'(\Xi)$.  Then, 
\bel{circular mean singularities}
 \WF(\Mst P \Mab f)\subset \paren{\WF(f)\cap \Vab}\cup \Aab(f).\ee
\end{theorem}

One would expect that an inclusion $\WF(f)\cap
\Vc_{(a,b)}\subset\WF(\Mst P \Mab f)$ holds, which is true for sonar,
as proven in Section \ref{sect:sonar}, and for limited angle x-ray
tomography with reconstruction operators considered in
\cite{FrikelQuinto2013}.  We will discuss why this is not possible, in
general, for the PAT transform in Remark \ref{remark:elliptic}.


\begin{remark}\label{remark:A and V}  In general, Radon transforms
detect singularities conormal to the set being integrated over, and so
the visible singularities should be conormal to circles in the data
set.  The set $\Vab$ is the collection of conormals to circles
$C(\phi,r)$ for $\phi\in [a,b]$, and, according to Theorem
\ref{thm:visible and added sing}, $\Vab\cap \WF(f)$ is the set of
possible visible singularities in $\Mst P \Mab f$.  This idea of
visible singularities being (co)normal to the manifold of integration
is well-known and is for example, discussed in \cite{Palamodov:JFAA,Quinto93}.  This follows from the pioneering work of Guillemin
\cite{Gu1975, GS1977} showing Radon transforms are FIO associated to a
conormal bundle.


There are also possible added singularities, $\Aab(f)$, and they come
about from the data at the limits of the angular range, $a$ and $b$.
Remarkably, if $f$ has a singularity at one point on the circle
$C(\phi,r)$ (for $\phi=a$ or $\phi =b$) conormal to the circle, then
that singularity can be spread over the entire circle in the
reconstruction.  

Figure \ref{fig:illustration of artifacts} illustrates this perfectly
(as do the reconstructions in Section \ref{sect:numerics}).  The data
are taken for $\phi\in [0,\pi]$.  Every singularity in $D$ is visible
since, for every $x\in D$ and $\xi\in \rtwo\smo$, there is a $\phi\in
[0,\pi]$ with $\xi=\alpha \n(\phi,x)$ for some $\alpha \neq 0$; that
is, for every covector $(x,\xi\dx)\in T^*(D)\smo$, there is a $\phi\in
[0,\pi]$ such that $(x,\xi\dx)$ is conormal to the circle
$C(\phi,\norm{x-\th(\phi)})$.

The added singularities are as predicted by the theorem. They appear
on circles $C(\phi,r)$ when $\phi = 0,\pi$, the endpoints of the
interval of detectors and when some singularity of $f$ is conormal to
the circle.  For the simple phantom in Figure \ref{fig:illustration of
artifacts} there are four circles of added artifacts, and they are
tangent to the boundary of the object at points on the horizontal
axis.
\end{remark}



Next, we will show that the same artifact reduction procedure suggested in
\cite{FrikelQuinto2013} is valid for this case, too.  Let $a'$ and
$b'$ be chosen so $a<a'<b'<b$ and choose a smooth cutoff function
$\vp:[0,2\pi]\to\rr$ supported in $(a,b)$ and equal to one on
$[a',b']$.  Define the operator $\Kvp:\Dc'(\Xi)\to \Dc'(\Xi)$ by
\bel{def:K}\Kvp g = \vp g.\ee Then $\Kvp \Mc$ uses only data for
$\phi\in [a,b]$ but it provides a smooth cutoff.  This discussion
leads to the following theorem.

\begin{theorem}[Reduction of Artifacts for the circular mean
transform]\label{thm:reduction:circle} Let $\Kvp$ be defined by
\eqref{def:K} and let $P$ be a pseudodifferential operator on
$\Ec'(\Xi)$.  Finally, let \[\Lvp = \Mst P \Kvp \Mc, \] then $\Lvp$ is
a standard smooth pseudodifferential operator.  So, if $f\in \Ec'(D)$,
then \bel{reduced WF} \WF(\Lvp(f))\subset \WF(f)\cap
\Vab.\ee\end{theorem} 

Thus, only visible singularities of $f$ are visible in $\Lvp(f)$, and
there are no added singularities.

The proofs of these theorems are in the appendix.

\begin{figure}
	\centering
	\includegraphics[width=4cm]{circ.png}\hskip1ex %\subfloat[Original]{}
	\includegraphics[width=4cm]{circ_lambda_0-180deg_CE_70-235}%\hskip1ex \subfloat[$\Lc^2 g$]{}
%	\subfloat[$\Ac_{\sparen{0,\pi}}$]
	\raisebox{-0.4pt}{
%	{
	\begin{tikzpicture}[scale=0.6667]
		% Lim angle sphere
		\draw [thick](-5cm,0) circle (0.75cm);
			
		% Rectangle
		\draw [thin, gray] (-8,-3) -- (-2,-3) -- (-2,3) -- (-8,3) -- (-8,-3);
			
		% Artifacts		
		\draw [dashed] (-7,3) arc (45:-45:4.25cm);
		\draw [dashed] (-5.1,3) arc (31.5:-31.5:5.75cm);
		\draw [dashed] (-3,3) arc (135:225:4.25cm);
		\draw [dashed] (-4.9,3) arc (148.5:211.5:5.75cm);
	\end{tikzpicture}
%	}
	}
	\caption{Lambda type reconstruction (middle) of the characteristic function of a circle (left) for the angular range $[0,\pi]$ and visualization of the set of added artifacts $\Ac_{\sparen{0,\pi}}$ (right). The correspondence between practical reconstruction and theoretical description \eqref{def:Aab} is remarkable.}
	\label{fig:illustration of artifacts}
\end{figure}

 \subsection{Sonar (spherical mean transform with centers on a
 plane)}\label{sect:sonar}

In this section, we analyze a limited data problem for sonar.  We
assume the sound speed is constant and there are not multiple
reflections.  Then, using the ansatz of Cohen and Bleistein
\cite{CB1979} the data can be reduced to integrals over spheres
centered on the ocean surface of the perturbation, $f(x)$, from the
constant sound speed.  We assume the ocean surface is planar and
consider sonar data from transceivers on a compact subset, $K$, of
that plane.

The functions we consider will be compactly supported in the open
upper half plane \[X:=\sparen{(x_1,x_2,x_3)\in \rthree\st x_3>0}.\]
Let $\Xis:= \rtwo\times (0,\infty),$ and denote the sphere centered at
$(y,0)$ and of radius $r$ by $S(y,r)=\sparen{x\in \rthree\st
\norm{x-(y,0)}=r}$.  The spherical mean transform of $f\in \Dc(X)$ is
denoted \bel{def:Ms}\Ms f(y,r) = \frac{1}{4\pi r^2}\int_{x\in
S(y,r)}f(x)\d x,\ee where $\d x$ is the surface measure on the sphere
$S(y,r)$.  For $g\in \Ec'(\Xis)$, the dual transform is given by 
\[\Msst g(x) = \int_{y\in \rtwo} g(y,\norm{x-(y,0)}) \frac{1}{4\pi
\norm{x-(y,0)}^2}\d y,\] where we note that the weight does not blow
up since the integral is evaluated at $x\in X$.

Let $K$ be a compact subset of $\rtwo$ with nontrivial interior.  We
consider the limited data problem where data are given over spheres
$S(y,r)$ with $(y,r)$ in \[A=K\times (0,\infty).\] The resulting
transform is \[\Msa = \chi_A \Ms.\] Since $K$ is compact, for any
$f\in \Ec'(X)$, $\Msa(f)\in \Ec'(\Xis)$.

For $x\in X$ and $y\in \rtwo$, we let \bel{def:nyx}\nyx =
\frac{x-(y,0)}{\norm{x-(y,0)}}\ee denote the outward unit normal at
$x$ to the sphere $S(y,\norm{x-(y,0)})$.  Note that the third
coordinate of $\nyx$ is never equal to zero since $x_3>0$. 

We define the set \bel{def:Vsk} \Vsk := \sparen{(x,\xi\dx)\in
T^*(X)\st \exists y\in K,\exists \alpha \neq 0, \xi = \alpha\nyx}.\ee
In our next theorem, we show $\Vsk$ is the set of \emph{possible
visible singularities}, i.e., those that can be imaged by $\Msst P
\Msa$ (singularities above points $y\in \bd(K)$ might be cancelled).

If $x=(x_1,x_2,x_3)\in \rthree$ then we define $x'=(x_1,x_2)$. 

Singularities are spread in more subtle ways in sonar than in TAT and
so we need to introduce more notation to properly describe these added
artifacts.  Let $S^2_+$ denote the open top hemisphere of $S^2$.  Let
$(y,r)\in \Xis$ and let $\eta\in \rtwo\smo$ and $\n\in S^2_+$.  Let
$C(y,r,\eta,\n)$ be the circle on $S(y,r)$ \bel{def:C}C(y,r,\eta,\n )
= \sparen{x\in S(y,r)\st \exists a\in \rr,\ x'-y=a\eta +r{\n'}}.\ee
This circle is the intersection of $S(y,r)$ with the vertical plane
that is parallel to $\eta$ and goes through $\paren{y+r\n',0}$. 

Let $K\subset\rtwo$ be a compact set bounded by a piecewise
$C^\infty$, simple, closed curve, $B=\bd(K)$.  Then, the singular
support of $\chi_K$ is $B$.  As noted in Example \ref{ex:char}, at
points $y\in B$ at which $B$ is a smooth curve, $(y,\eta\dy)\in
\WF(\chi_K)$ if and only if $\eta$ is normal to $B$ at $y$.  On the
other hand, if $B$ has a corner at $y$ then all covectors above $y$
are in $\WF(\chi_K)$. By \cite{Petersen}, $\WF(\chi_K)$ is a set
of covectors above $\bd(K)$, and at any point $y\in \bd(K)$ at which
$\bd(K)$ is smooth, they are the conormal covectors to $\bd(K)$ at
$y$ (see the discussion in Example \ref{ex:char}).  

The following definition allows us to apply our next theorem to more
general sets $K$ than those with piecewise smooth boundaries.

\begin{definition}[Generalized Normal Bundle] \label{def:generalized
normal bundle} Let $K$ be a compact subset of $\rtwo$.  Define
\emph{the generalized normal bundle of $K$ to be the set, $N(K)$, of
vectors in $\rtwo\times \paren{\rtwo\smo}$ corresponding to  covectors in the
wavefront set of $\chi_K$: }
\[N(K) = \sparen{(y,\eta)\in \rtwo\times \paren{\rtwo\smo}\st (y,\eta\dy)\in \WF(\chi_K)}.\]
\end{definition}

Using this notation and with $A=K\times (0,\infty)$, the wavefront set
of $\chia$ as a function on $\Xi_\Sc$ is \[\WF(\chia) =
\sparen{((y,r),\eta\dy)\st (y,\eta)\in N(K), r>0}.\] 

If $K$ is bounded by a smooth closed curve then our definition of
$N(K)$ corresponds with the standard definition of the normal bundle
of $\bd(K)$. However, if $K$ itself is a curve, then $\chi_K=0$ as a
distribution.  This means that, by our definition $N(K)=\emptyset$,
and this definition does not exactly correspond to the standard normal
bundle of $\bd(K)=K$.

Now, we introduce the set of added singularities. Let $f\in \Ec'(X)$
and let $K$ a compact subset of $\rtwo$.  Define the set
\bel{def:Ask}\begin{aligned} \Ask(f):=&\bigcup
\Big\{\big\{(x,\alpha\n(y,x)\dx) \st x\in
C(y,r,\eta,\n(y,\tx))\big\}\\&\qquad \st (y,\eta)\in N(K),\ r>0,\
\alpha\neq 0,\ \tx\in S(y,r)\ \text{ and
}\paren{\tx,\alpha\n(y,\tx)\dx}\in WF(f)\Big\}.\end{aligned}\ee


We will say more about this set
after the theorem. 

\begin{theorem}[Visible and Added Singularities for the Spherical
transform]\label{thm:visible and added sing sphere} Let $f\in \Ec'(X)$
and let $P$ be a properly supported pseudo\-differential operator on
$\Dc'(\Xi_{\Sc})$.  Let $K$ be a compact subset of $\rtwo$ with
nontrivial interior and let and $A=K\times (0,\infty)$.  Then,
\bel{spherical mean singularities} \WF(\Msst P \Msa f)\subset
\paren{\WF(f)\cap \Vs{K}}\cup \As{K}(f).\ee If $P$ is elliptic on
$\range(\Ms)$, then,
\bel{elliptic spherical}
\WF(f)\cap\Vs{\intt(K)}\subset
\WF(\Msst P \Msa f)\,.\ee
\end{theorem}


\begin{remark}\label{remark:wild singularities}
In practice, $K$ will be a compact set bounded by a simple piecewise
smooth curve, and we now consider $\Ask(f)$ in this case.  By the
definition of $\Ask(f)$ and Theorem \ref{thm:visible and added sing
sphere}, singularities are added on spheres $S(y,r)$.  For added
singularities to appear on $S(y,r)$ the following must be satisfied:
\begin{itemize}
\item $y\in \bd(K)$

\item There is an $\tx\in S(y,r)$ and $\alpha \neq 0$ with
$(\tx,\alpha\n(y,\tx))\in \WF(f)$.

\end{itemize}
Once this is true, the singularities spread differently depending on
the geometry of $\bd(K)$.  Let $y\in \bd(K)$, $r>0$, and $\alpha\neq
0$.  Assume $\tx\in S(y,r)$ with $(\tx,\alpha\n(y,\tx)\dx)\in \WF(f)$.


First, assume $\bd(K)$ is a smooth curve at $y$.  Let $\eta$ be a
normal to $\bd(K)$ at $y$, then all normals to $\bd(K)$ at $y$ are
parallel to $\eta$.  Thus, the added singularities caused by the
singularity of $f$ at $(\tx,\alpha\n(y,\tx)\dx)$ will be on the
semicircle $C(y,r,\eta,\alpha\n(y,\tx))\cap X$ but nowhere else on
$S(y,r)$.

Now assume that $\bd(K)$ has a corner at $y$.  Then, for all $\eta\neq
0$,$(y,\eta)\in N(K)$.  Each such $\eta$ generates a semicircle of
possible added singularities that is in a plane parallel to $\eta$ and
through the fixed point $(y+r\n'(y,\tx),0)$.  As $\eta$ changes, this
semicircle sweeps out the entire hemisphere $S(y,r)\cap X$. Thus, in
this case, added singularities are on this entire hemisphere.

This discussion justifies using measurement sets $K$ with smooth
boundaries so added singularities do not spread along entire
hemispheres.
\end{remark}

These theorems do not address what happens to ``boundary
singularities'' of $f$, namely those for covectors $(x,\xi\dx)\in
\Vc_{\bd(K)}$.  In general, these singularities can be invisible or
visible.


The reconstruction from simulated sonar data in Figure
\ref{fig:QRS2011}, which was taken from \cite{QRS2011}, illus\-trate
our theorem perfectly; there are added singularities in exactly the places
predicted by the theorem.  In fact, all of the reconstructions in
\cite{QRS2011} have the added artifacts in the locations predicted by
the theorem.
\begin{figure}[ht]
\centerline{
\includegraphics[width=5cm]{ballsFig2-3-QRS2011.png}}
\caption{Reconstruction from spherical mean data of the characteristic
functions of two balls and a horizontal ocean floor.  The center set
$K=[-12,12]^2$ and the reconstruction is in the plane $x_1=0.25$. The
spheres are centered at $(0,0,3)$ and $(0,1,4)$. The added artifacts
in this picture are along circles parallel the $x_2\,x_3$ plane (since
they are caused by normals perpendicular to the $x_1$ axis for spheres
centered on lines parallel the $x_1$ axis).  Note that the predicted
artifact caused by the ocean floor would be outside the reconstruction
region since it would be caused by spheres centered at $(0.25,\pm
12,0)$ and of radius 6.  Reprinted from \cite{QRS2011} by permission
of IOP Publishing.} \label{fig:QRS2011}
\end{figure}



The same artifact reduction procedure suggested in
\cite{FrikelQuinto2013} is valid for this case, too.  Let $K'$ be an
open set whose closure is contained in $\intt(K)$ and let
$\vp:\rtwo\to\rr$ be a smooth cutoff function that is supported in
$\intt(K)$ and equal to one on $K'$. In this case, the operator
$\Kvp:\Dc'(\Xi_{\Sc})\to \Dc'(\Xi_{\Sc})$ is
\[\Kvp g = \vp g.\] Then $\Kvp \Ms$ uses only data for
$y\in K$ but it provides a smooth cutoff.  This discussion leads to
the following theorem.

\begin{theorem}[Reduction of Artifacts for the sonar
transform]\label{thm:reduction:sphere} Let $K$ be a compact subset of
$\rtwo$ with nontrivial interior.  Let $P$ be a properly supported
pseudodifferential operator on $\Ec'(\Xi_{\Sc})$.  Let $K'$ be an open
set whose closure is contained in $\intt(K)$ and let $\vp:\rtwo\to\rr$
be a smooth function supported in $\intt(K)$ and equal to one on $K'$.
Let \[\Lvp = \Msst P \Kvp \Ms, \] then $\Lvp$ is a standard $C^\infty$
pseudodifferential operator and so 
\[\WF(\Lvp(f))\subset \WF(f)\cap \Vsk\] for $f\in \Ec'(X)$.  If $P$ is
elliptic on $\range(\Ms)$, then $\Lvp$ is
elliptic on $\Vs{K'}$, so, if $f\in \Ec(D)$, then \bel{reduced WF}
\WF(f)\cap \Vs{K'}\subset\WF(\Lvp(f))\subset \WF(f)\cap \Vsk.
\ee\end{theorem} 

Thus, only visible singularities of $f$ are visible in $\Lvp(f)$, and
there are no added singularities.  In contrast to the circular mean
case, when $P$ is elliptic, all of the singularities of $f$ in
$\Vs{K'}$ are visible in $\Lvp( f)$.  This difference will be
explained in Remark \ref{remark:elliptic}.



==> theoremenv.tex <==
%------------- Theorem Environments -------------
\usepackage[amsmath,standard,thmmarks]{ntheorem}
%\usepackage{amsthm}
%\qedsymbol{\diamondsuit}


%%\theorembodyfont{\rmfamily}
%\theoremnumbering{arabic}
%%\theoremindent0.5cm

%\theoremstyle{break}

\makeatletter
\newtheoremstyle{mythm}%
{\item[\hskip\labelsep \theorem@headerfont ##1\ ##2\theorem@separator]}%
{\item[\hskip\labelsep \theorem@headerfont ##1\ ##2\ \normalfont{(##3)}\theorem@separator]}
\makeatother

\theoremstyle{mythm}
\theoremseparator{.}

\renewtheorem{Proof}{Proof}

\renewtheorem{theorem}{Theorem}[section]
\renewtheorem{lemma}[theorem]{Lemma}
\renewtheorem{corollary}[theorem]{Corollary}
\renewtheorem{proposition}[theorem]{Proposition}
\newtheorem{assumption}{Assumption}[section]

\renewtheorem{definition}[theorem]{Definition}

\theorembodyfont{\rmfamily}
\newtheorem{algorithm}[theorem]{Algorithm}


%\theoremstyle{break}
\theoremstyle{nonumberbreak}
\theoremheaderfont{\itshape}
\renewtheorem{example}{Example}
\renewtheorem{remark}{Remark}

\theoremstyle{nonumberbreak}
\newtheorem{remarks}[theorem]{Remarks}
\newtheorem{examples}[theorem]{Examples}

\makeatletter
\newtheoremstyle{myproof}%
{\item[\hskip\labelsep \theorem@headerfont ##1\theorem@separator]}%
{\item[\hskip\labelsep \theorem@headerfont ##1\ ##3\theorem@separator]}
\makeatother

\theoremstyle{myproof}
\theoremheaderfont{\bfseries}%{\slshape}\itshape %\scshape
\theoremseparator{.}
\theoremsymbol{\hbox{}\hfill {\tiny$\blacksquare$}}%{\hfillensuremath{\diamondsuit}}
\renewtheorem{Proof}{Proof}
\renewtheorem{proof}{Proof}
%------------------------------------------------
